Improved Linear Embeddings via Lagrange Duality

Near isometric orthogonal embeddings to lower dimensions are a fundamental tool in data science and machine learning. In this paper, we present the construction of such embeddings that minimizes the maximum distortion for a given set of points. We formulate the problem as a non convex constrained optimization problem. We first construct a primal relaxation and then use the theory of Lagrange duality to create dual relaxation. We also suggest a polynomial time algorithm based on the theory of convex optimization to solve the dual relaxation provably. We provide a theoretical upper bound on the approximation guarantees for our algorithm, which depends only on the spectral properties of the dataset. We experimentally demonstrate the superiority of our algorithm compared to baselines in terms of the scalability and the ability to achieve lower distortion.

==> intro.tex <==
One of the fundamental tool used in data science and machine learning is Johnson-Lindenstrauss ({\em JL} for short) transformation which allows embedding of the high-dimensional data points into lower dimensional space in such a way that distances between the points are nearly preserved. The mathematical theory behind such a transformation was developed by  William B. Johnson and Joram Lindenstrauss in 1984~\cite{Johnson84} and the precise statement is popularly known as JL Lemma.
\begin{theorem}[Johnson-Lindenstrauss Lemma~\cite{Johnson84}] For any $0<\epsilon<1$ and any integer $n>1$, let $k$ be a positive integer such that $k \ge C \epsilon^{-2} \ln n$, where $C$ is a suitable constant. Then for any set $S$ of $n$ points in $\mathbb{R}^d$, there exists a linear map $f \mapsto \mathbb{R}^d \rightarrow \mathbb{R}^k$ such that for all $\boldsymbol{u},\boldsymbol{v} \in S$,
\begin{eqnarray}
(1-\epsilon) \lVert \boldsymbol{u} - \boldsymbol{v} \rVert^2 \le \lVert f(\boldsymbol{u}) - f(\boldsymbol{v})\rVert^2 \le (1 + \epsilon)\lVert \boldsymbol{u} - \boldsymbol{v} \rVert^2.
\end{eqnarray}
\end{theorem}
The remarkable fact about this lemma is that the dimension of the lower dimensional space $k$ is independent of the original dimension $d$ and depends only on the logarithmic of the size of the data and the error parameter $\epsilon$, i.e., $k = O(\frac{1}{\epsilon^2}\ln n)$. Furthermore, Also, the One of the key fact behind the widespread applicability of the J-L lemma in computer science is that it can be viewed as a compression scheme which helps to reduce significantly the space required for storing multidimensional data~\cite{Johnson10}. 

As mentioned in \cite{Matousek08}, all known proofs of the the JL Lemma proceed according to the following generic scheme - For given $n$ and $k$, one defines a suitable probability distribution $\mathcal{F}$ over the set of all linear maps $T: \mathbb{R}^d \mapsto \mathbb{R}^k$. Then one proves the following statement.
\begin{statement} If $T: \mathbb{R}^d \mapsto \mathbb{R}^k$ is a random linear mapping drawn from the distribution $\mathcal{F}$, then for every point $\boldsymbol{x} \in \mathbb{R}^d$, we have
\begin{eqnarray}
Pr\left[\;(1-\epsilon) \lVert x\rVert^2 \le \lVert T(x) \rVert^2 \le (1+\epsilon)\lVert x \rVert^2 \; \right] \ge 1- \frac{1}{n^2}
\end{eqnarray}  
\end{statement}
Having established such a statement for the considered distribution $\mathcal{F}$, the proof of JL Lemma becomes quite easy. For this, one essentially uses probability union bound and $\boldsymbol{x}=(\boldsymbol{u}-\boldsymbol{v})$ to show that if  $T: \mathbb{R}^d \mapsto \mathbb{R}^k$ is a random linear mapping drawn from the distribution $\mathcal{F}$ then we have
\begin{comment}
\begin{eqnarray}
\begin{split}
Pr[\;\forall (\boldsymbol{u},\boldsymbol{v})\in S, \(1-\epsilon) \lVert \boldsymbol{u} - \boldsymbol{v} \rVert^2 & \le \lVert T(\boldsymbol{u}) - T(\boldsymbol{v}) \rVert^2 \\
& \le (1+\epsilon)\lVert \boldsymbol{u} - \boldsymbol{v} \rVert^2 \; ] > 1/2
\end{split}
\end{eqnarray}
\end{comment}
which proves the existence of desired linear map. In the original proof~\cite{Johnson84}, the support of the distribution $\mathcal{F}$ was the set of all the orthogonal projections going from $\mathbb{R}^d$ to $\mathbb{R}^k$ multiplied with a scaling factor of $\sqrt{d/k}$. Intuitively, they randomly selected an orthogonal project matrix, say $\mathbf{V}$ of size $k \times d$ and then transformed every vector $\boldsymbol{x}\in \mathbb{R}^d$ as $\sqrt{d/k}\mathbf{V}\boldsymbol{x}$. Note, length of the vector $\mathbf{V}\boldsymbol{x}$ is at most the length of the vector $\boldsymbol{x}$ because of orthogonal projection. This construction allows to write the following alternate statement of the JL lemma (known as distributional JL Lemma)~\cite{Chen15}.
\begin{theorem}[Distributional JL Lemma] For any given $0 < \epsilon, \delta < 1/2$ and a positive integer $d$, there exists a distribution $\mathcal{F}$ over linear maps from $\mathbb{R}^d$  to $\mathbb{R}^k$ (i.e. set of all $k \times d$ sized matrices) such that for $k = O(\frac{1}{\epsilon^2}\ln (1/\delta))$ if we randomly draw a matrix $\mathbf{V}$ from distribution $\mathcal{F}$ then for any unit length vector $\boldsymbol{x}\in \mathbb{R}^d$ we must have
\begin{eqnarray}
Pr\left[\; \lvert 1- \lVert\mathbf{V}\boldsymbol{x}\rVert ^2\rvert  > \epsilon \;\right] < \delta
\end{eqnarray}
\end{theorem}
An interesting fact about this version of JL Lemma is that for any appropriately chosen distribution $\mathcal{F}$, a random projection matrix preserves the length of any unit vector with high probability and moreover, this matrix is {\bf oblivious to the data set $S$}. If a prior information of $S$ is known~\cite{Chen15}, one may find a better mapping which is adapted to $S$. This observation is precisely the starting point and the motivation behind the problem considered in this paper.     


==> old_methods.tex <==
\begin{comment}
As mentioned in the previous section, the motivation behind studying the problem in this paper stems from its connection with JL transformation that preserves the lengths of unit vectors when projected into an appropriate lower dimensional linear subspace. The linear transformation map suggested in the original work of Johnson and Lindenstrauss \cite{Johnson84} was (i) a scaled orthogonal projection, (ii) probabilistic in nature, and (iii) data oblivious. Later developments suggested a randomly chosen subspace into which data are projected (not necessarily orthogonally) so that the squared projected length of the unit vector lies in $(1 \pm \epsilon)$. Such schemes (see ~\cite{Matousek08, Chen15} for details) also have theoretical lower bounds on the dimension of the space into which data can be projected and that is proportional to $1/\epsilon^{2}$. 



In this paper, we ask and try to answer a slightly different yet related question:

{\em What if we choose a linear transformation for the given set of data (in the form of unit vectors) such that the transformation is (i) an orthogonal projection, (ii) deterministic, and (iii) data non-oblivious (i.e. data adaptive); and further, project the given set of unit vector data using this transformation?} 

Note, each such transformation can be identified with a unique linear subspace of $\mathbb{R}^d$ and moreover, each such transformation can only decrease the length of any given unit vector. Therefore, under such a transformation, for the purpose of preserving lengths of the unit vectors in set $S$, we must strive to maximize the minimum length of the projected vectors. Thus, unlike JL lemma -- where error parameter $\epsilon$ is specified by the user and an appropriate $k$ is determined accordingly -- in our version of the problem, we start with a $k$ and search across all possible $k$ dimensional subspaces to identify a subspace that preserves the lengths of given set of unit vectors, under orthogonal projection, upto the maximum extent. A natural way to quantify the extent to which distances are being preserved is to consider the minimum length (or, {\em equivalently minimum squared length}) of projected vectors and our goal should be to maximize this. We call this problem as {\em Adaptive JL Transformation (AJLT)}. In what follows, we present a mathematical formulation for the same.
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%----------------------------------- AJLT Formulation ----------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Problem Formulation}
Let $\{\boldsymbol{u_i}\}_{i=1}^r$ be a given dataset where $\boldsymbol{u_i} \in \mathbb{R}^d$ $\forall$ $i \in [r]$. As mentioned in the previous section, our goal is to orthogonally project (aka embed) these data into a subspace of dimension $k$. Because the projection is linear as well as orthogonal, the required condition for near isometric embedding becomes
\[1- \epsilon \leq \frac{\|\mathbf{P}(\boldsymbol{u_i} - \boldsymbol{u_j}) \|_2^2}{\|\boldsymbol{u_i} - \boldsymbol{u_j}\|_2^2}\;\;\;\forall i < j \in[r] \] 
where, $\mathbf{P}$ is the required linear map. 
In light of this inequality, we do the following - compute normalized pairwise differences given by $\left(\boldsymbol{u_i} - \boldsymbol{u_j}\right)/\lVert\left(\boldsymbol{u_i} - \boldsymbol{u_j}\right)\rVert$ for every pair $(i,j)$, where $i <j; (i,j) \in[r]$, and then orthogonally project them to preserve their squared lengths. This way, we get $r \choose 2$ vectors each being unit length. If we let $n = {r \choose 2}$ then, we can denote such vectors by $\boldsymbol{x}_1, \boldsymbol{x}_2, \ldots, \boldsymbol{x}_n$ and our goal becomes to orthogonally project them so as to preserve their squared lengths.
%Let set $S$ comprises these $n$ unit length vectors in a $d$-dimensional Euclidean space, denoted by  , which are pairwise unit norm differences. 
For this, we let $\boldsymbol{v}_1\neq0, \boldsymbol{v}_2\neq0,\ldots, \boldsymbol{v}_k\neq0$ be some orthogonal basis vectors of a $k$-dimensional subspace ${\mathcal{S}}_k$ of $\mathbb{R}^d$.  Further, let $\mathbf{V}$ be a $d \times k$ matrix whose columns are given by the orthogonal basis vectors $\boldsymbol{v}_1, \boldsymbol{v}_2,\ldots, \boldsymbol{v}_k$. Let  $\boldsymbol{\tilde{x}}_i \in {\mathcal{S}}_k$ be the vector obtained by projecting $\boldsymbol{x}_i$ orthogonally into the space ${\mathcal{S}}_k$. Then, the problem of pushing the lower bound in inequality (\ref{JL_Inequality}) as close to $1$ as possible is equivalent to minimizing a real number $\text{\LARGE{$\epsilon$}}$ such that the distortion of each of the $x_i$'s after projection is less than $\text{\LARGE{$\epsilon$}}$. Here, the distortion is given by the squared length of the residual vector $(\boldsymbol{{x}}_i-\boldsymbol{\tilde{x}}_i)$, which would be equal to $1-\lVert \boldsymbol{\tilde{x}}_i\rVert^2$. Formally, it can be stated as the following optimization problem which we refer to as the \textbf{Primal} problem.
\rule{\columnwidth}{0.5pt}
\vspace{-0.5cm}
 \begin{align}
 &\underset{\boldsymbol{v}_1\neq0,\ldots,\boldsymbol{v}_k \neq0, \text{\large{$\epsilon$}}}{\text{Minimize }}\text{\LARGE{$\epsilon$}}\nonumber\\
 & \text{subject to}\ \ 1- \lVert \mathbf{V}^{\top} \boldsymbol{x}_i \rVert_2^2\le \text{\LARGE{$\epsilon$}},\;\forall i =1,\ldots, n\nonumber\\
& \boldsymbol{v}_j^{\top}\boldsymbol{v}_j = 1,\;\forall j =1,\ldots, k\nonumber\\
& \boldsymbol{v}_j^{\top}\boldsymbol{v}_m = 0,\;\forall j  \neq m \eqname{(Primal)} \label{Primal}
 \end{align} 
%\vspace{-0.5cm}
\rule{\columnwidth}{0.5pt}

 The last two constraints force the matrix $\mathbf{V}$ to be orthonormal. The first constraint, on the other hand, identifies the vector for whom $1- \lVert \boldsymbol{\tilde{x}}_i \rVert^2$ is maximum. 
 %or equivalently $\lVert \boldsymbol{\tilde{x}}_i \rVert^2$ is minimum. 
 The objective function tries to minimize  $1- \lVert \boldsymbol{\tilde{x}}_i \rVert^2$ for such a vector. 
 Observe, whenever $\mathbf{V}$ is an orthogonal matrix, we have $\lVert \boldsymbol{\tilde{x}}_i \rVert^2 = \lVert \mathbf{V}^{\top} \boldsymbol{x}_i \rVert^2 \le 1$ for each $i=1,\ldots,n$. 
%which is equivalent to maximizing  the minimum length (or minimum squared length) of any projected vector.     
%\begin{eqnarray}
%\lVert \boldsymbol{x}_i - {\boldsymbol {\tilde {x}}}_i \rVert_2^2 &=& 1 - \lVert\ {\boldsymbol {\tilde {x}}}_i \rVert_2^2 \nonumber\\
%&=& 1- \lVert \mathbf{V}\mathbf{V}^{\top} \boldsymbol{x}_i \rVert_2^2
%\end{eqnarray}
%$In view of the above relation, Min-Max PCA can be expressed by means of the following equivalent formulation. We call this as {\em Primal} problem for the reasons that would become clear soon.

Let $p^*$ be the optimal value of the above problem. It is straightforward  to verify that $0 \le p^* \le 1$. 
\begin{comment}


\subsection{Near Isometric Orthogonal Linear Embeddings}

In this section, we discuss our approach to approximately solve the \ref{Primal} problem where we formulate and solve the Lagrangian dual of its relaxed version and the dual turns out to be a convex program. Our Lagrangian duality based relaxation of the non-convex \ref{Primal} problem has much less number of constraints and that allows us to come up with a computationally efficient algorithm for solving the \ref{Primal} problem. The details of our approach is given in the next section. 
\end{comment}
\subsection{Lagrangian Dual}
The \ref{Primal} problem is a non-convex optimization problem as the feasible region forms a non-convex set. So we cannot hope to exactly solve this problem efficiently and hence we aim for approximate solutions.

For this, we momentarily ignore the the last equality constraint in \ref{Primal} problem, which enforces orthogonality of the $v_j$'s, and consider the following {\em Relaxed Primal} problem. We will later prove that inspite of this relaxation, we will reach a solution in which the vectors are indeed orthogonal, thereby satisfying the constraints of the \ref{Primal} problem and justifying the effectiveness of our approach.\\
\rule{\columnwidth}{0.5pt}
\vspace{-0.5cm}
\begin{align*}
&\underset{\boldsymbol{v}_1\neq0,\ldots,\boldsymbol{v}_k\neq 0 , \text{$\epsilon$}}{\text{Minimize }} \text{\LARGE{$\epsilon$}}\\
& \text{subject to} \ \ 1- \lVert \mathbf{V}^{\top} \boldsymbol{x}_i \rVert_2^2\le \text{\LARGE{$\epsilon$}},\;\forall i =1,\ldots, n\nonumber\\
& \boldsymbol{v}_j^{\top}\boldsymbol{v}_j = 1,\;\forall j =1,\ldots, k \eqname{(Relaxed Primal)} \label{Relaxed_Primal}
\end{align*} 
\rule{\columnwidth}{0.5pt}
The following lemma is going to be useful in subsequent developments, we omit the proof as it is fairly straightforward.
\begin{lemma} \label{lemma1}Let $\widehat{p^*}$ is the optimal value of the \ref{Relaxed_Primal} problem. Then, followings hold true.
\begin{enumerate}[label=(\Alph*)]
\item $\widehat{p^*} \le p^* \le 1$.
\item If an optimal solution of the \ref{Relaxed_Primal} problem satisfies the constraints of the \ref{Primal} problem then that solution must be an optimal solution for the  \ref{Primal} problem also.
\end{enumerate}
\end{lemma}
Note, the constraint $\boldsymbol{v}_j^{\top}\boldsymbol{v}_j = 1$ forces both \ref{Primal} as well as \ref{Relaxed_Primal} problems to be non-convex. The reason being following - {\em any norm is a convex function and the level set of a norm is a non-convex set}.  This motivates us to work with the Lagrangian dual of the \ref{Relaxed_Primal} problem and develop a strategy to get an approximate solution of the original \ref{Primal} problem.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------------------AJLT Dual Formulation-------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \subsection{Dual of Relaxed Primal} 
The Lagrangian dual for \ref{Relaxed_Primal} will always be a convex program irrespective of convexity of the \ref{Relaxed_Primal}. For this, we write down the Lagrangian function of \ref{Relaxed_Primal} as follows:
\begin{align}
& L(\boldsymbol{v}_1,\ldots,\boldsymbol{v}_k,\;\text{\LARGE{$\epsilon$}},\; \lambda_1,\ldots,\lambda_n,\mu_1,\ldots,\mu_k) \nonumber \\
& = \text{\LARGE{$\epsilon$}} + \sum_{i=1}^{n} \lambda_i \left(1- \lVert \mathbf{V}^{\top} \boldsymbol{x}_i \rVert_2^2 - \text{\LARGE{$\epsilon$}}\right) 
+ \sum_{j=1}^{k} \mu_j \left(\boldsymbol{v}_j^{\top} \boldsymbol{v}_j - 1\right)  
%\label{Lagrangian} \eqname{(Lagrangian)}
\end{align}
Observe, $\boldsymbol{v}_1,\ldots,\boldsymbol{v}_k,\;\text{\LARGE{$\epsilon$}}$ are the primal variables and
$\lambda_1,\ldots,\lambda_n,\mu_1,\ldots,\mu_k$ are the dual variables. The dual function is given by
\begin{align*}
g(\boldsymbol{\lambda},\boldsymbol{\mu})=\underset{\boldsymbol{v}_1\neq,\ldots,\boldsymbol{v}_k\neq0,\text{\large{$\epsilon$}}}{\text{argmin}} L(\boldsymbol{v}_1,\ldots ,\boldsymbol{v}_k,\text{\LARGE{$\epsilon$}},\lambda_1,\ldots \lambda_n,\mu_1,\ldots,\mu_k) 
\end{align*}
For any set of values $\{\lambda_i, \lambda_i \ge 0\}$, we define matrix 
$M=\sum_{i=1}^{n} \lambda_i \boldsymbol{x}_i\boldsymbol{x}_i^{\top}=\mathbf{X}^{\top}diag(\lambda_1,\ldots,\lambda_n) \mathbf{X}$.
The following lemma characterizes the dual solution in terms of this matrix $M$. 

%--------------------------------------------------------------------------------------------
\begin{lemma} \label{dual_lemma} Define $M=\sum_{i=1}^{n} \lambda_i \boldsymbol{x}_i\boldsymbol{x}_i^{\top}=\mathbf{X}^{\top}diag(\lambda_1,\ldots,\lambda_n) \mathbf{X}$. Then for any given values of dual variables $(\lambda_1,\ldots,\lambda_n,\mu_1,\ldots,\mu_k)$, $\lambda_i \ge 0$, we have
 \begin{align*}
 g(\boldsymbol{\lambda},\boldsymbol{\mu}) = \begin{cases}
                                              1-\sum\nolimits_{j=1}^{k} \mu_j :\text{If }\sum_{i=1}^{n}\lambda_i=1 \text{ and } \{\mu_j\}_{j=1}^{k}\\
                                              \ \text{ are the} \text{ top-$k$ eigenvalues of } M\\
                                              -\infty \text{ or  undefined}: \text{Otherwise}
                                            \end{cases}
 \end{align*}   
 Furthermore,the top-$k$ eigenvectors of the matrix $M$ are the minimizers of Lagrangian function. 
 \end{lemma}
 %--------------------------------------------------------------------------------------------
\begin{proof}
In order to get the dual function, we set the gradient of Lagrangian function (with respect to primal variables) to be zero. This gives us the following conditions.
\begin{eqnarray}
{\partial L}/{\partial \boldsymbol{v}_j} &=& 2 \mu_j\boldsymbol{v}_j - 2 \left(\sum\nolimits_{i=1}^{n} \lambda_i \boldsymbol{x}_i\boldsymbol{x}_i^{\top}\right)\boldsymbol{v}_j=0 \label{Lagrangian_Partial1}\\
{\partial L}/{\partial \text{\LARGE{$\epsilon$}}} &=& 1-\sum\nolimits_{i=1}^{n} \lambda_i =0 \label{Lagrangian_Partial2}
\end{eqnarray}
%The above equations mean that $\sum\nolimits_{i=1}^{n} \lambda_i=1$ and each $(\mu_j,\boldsymbol{v}_j)$ is some eigenvalue eigenvector pair of $M$. Now we will show that if $\sum\nolimits_{i=1}^{n} \lambda_i\neq1$ or if $\mu_j$ is not the top $j^{th}$ eigenvalue of $M$ then with some assignment of the primal variables we can drive the lagrangian function to $-\infty$ which does not make sense (\textbf{"Please make changes here and incorporate techinical wording"}).\\
Using the definition of matrix $M$, we first rewrite the expression for Lagrangian as follows.
 \begin{align}
 & L= \text{\LARGE{$\epsilon$}} \left(1-\sum\nolimits_{i=1}^{n} \lambda_i\right) + \sum\nolimits_{i=1}^{n} \lambda_i -\sum\nolimits_{j=1}^{k}\mu_j \nonumber\\
 &  - \sum\nolimits_{j=1}^{k} \boldsymbol{v}_j^{\top} \left(M - \mu_j \mathbf{I}\right)\boldsymbol{v}_j 
 %\label{Lagrangian_alternate} \eqname{(Lagrangian)}
 \end{align}
 The minimum value of the Lagrangian has to satisfy the first order conditions that we get by 
 setting the gradient of Lagrangian function (with respect to primal variables) to be zero. This gives us the following conditions.
\begin{align}
{\partial L}/{\partial \boldsymbol{v}_j} &= 2 \mu_j\boldsymbol{v}_j - 2 \left(\sum\nolimits_{i=1}^{n} \lambda_i \boldsymbol{x}_i\boldsymbol{x}_i^{\top}\right)\boldsymbol{v}_j=0 \label{Lagrangian_Partial1}\\
{\partial L}/{\partial \text{\LARGE{$\epsilon$}}} &= 1-\sum\nolimits_{i=1}^{n} \lambda_i =0 \label{Lagrangian_Partial2}
\end{align}
By looking at these conditions, the following claims follow.
 \begin{enumerate}
 \item As per equation \eqref{Lagrangian_Partial2}, $\sum_{i=1}^n\lambda_i = 1$. This can also equivalently be argued as the following:
 since $\LARGE{\epsilon}$ is unconstrained, if $\sum_{i=1}^n\lambda_i \neq 1$, then it is possible to set $\LARGE{\epsilon}$ such that
  $g(\boldsymbol{\lambda},\boldsymbol{\mu}) = -\infty$. 
  
 
 \item  Equation~\eqref{Lagrangian_Partial1} implies that for achieving minimum, the primal variables $\boldsymbol{v}_j $ must be an eigenvector of the 
 matrix $M=\sum_{i=1}^{n} \lambda_i \boldsymbol{x}_i\boldsymbol{x}_i^{\top}$ whose corresponding eigenvalue is
 the dual variable $\mu_j$. 
 
 We argue that setting $\mu_j$ to be any value other than the top-$j^{th}$ eigenvalue of the $M$
 leads to $g(\boldsymbol{\lambda},\boldsymbol{\mu})$ being either $-\infty$ or undefined. For this, note that under the condition given by \eqref{Lagrangian_Partial2}, Lagrangian becomes 
 \begin{align*}
 1-\sum\limits_{j=1}^{k} \mu_j - \sum\limits_{j=1}^{k} \boldsymbol{v}_j^{\top} \left(M - \mu_j \mathbf{I}\right)\boldsymbol{v}_j
 \end{align*}

 
 Without loss of generality, we can assume that $\mu_1 \ge \mu_2 \ge \ldots \ge \mu_k$. 
 Suppose $\gamma_1\ge \gamma_2 \ge \ldots \ge \gamma_d$ are the eigenvalues of the  the matrix $M$. 
 For contradiction assume that $\mu_1$ is not an eigenvalue of the matrix $M$. Now, let us consider two different cases.
 \begin{enumerate}
 \item {\bf Case of [$\mathbf{\gamma_1  > \mu_1}$]:} In this case, we can assign $\boldsymbol{v}_1 $ to be scaled eigenvector corresponding to the eigenvalue $\gamma_1$ and that would drive the Lagrangian value towards $-\infty$. Therefore, in order to avoid the $-\infty$ value for the dual function, we must have $\mu_1 \ge \gamma_1$.
 \item {\bf Case of [$\mathbf{\mu_1  > \gamma_1}$]:}  Under this scenario, we again consider two subcases:
 \begin{enumerate}
 \item {\bf Subcase of [$\mathbf{\gamma_1  > \mu_k}$]:} In such a case, by the previous argument, we can again drive the Lagrangian to $-\infty$ by assigning $\boldsymbol{v}_k$ appropriately. 
 \item {\bf Subcase of [$\mathbf{\mu_k > \gamma_1}$]:} For this subcase, note that matrix $\left(M - \mu_j \mathbf{I}\right)$ would be a negative definite matrix for each $j \in[k]$ and 
 hence $\boldsymbol{v}_j=0,\;\forall j \in [k]$ will minimize the Lagrangian. However, all $v_j$ cannot simultaneously be zero as per the constraint.
 Hence, in this case, the minimum is not defined within the (open) set of $\{v_j ,\; \forall j\ v_j \neq 0 \}$. 
 
% However, we cannot take all $\boldsymbol{v}_j=0,\;\forall j \in [k]$ because the definition of the dual problem doesn't allow such an assignment. "\textbf{Please add technical wording for infeasibiliy of dual variables here}".      
 \end{enumerate}
 \end{enumerate}
Thus, we can conclude that $\mu_1$ should be equal to $\gamma_1$ in order to make sure that the dual
function is well defined and has a finite value. 
This also means that $v_1$ has to be the top eigenvector of $M$. We can inductively apply the same argument for other $\mu_j$ also to get the desired claim.
 \end{enumerate}
 \end{proof} 
Lemma \ref{dual_lemma} suggests that  the vectors  $\boldsymbol{v}_1 \neq 0,\ldots, \boldsymbol{v}_k \neq 0$ which minimize Lagrangian must be the top-$k$ eigenvectors of the matrix $M$ and in such a case, the dual function can be given as follows $g(\boldsymbol{\lambda},\boldsymbol{\mu}) = 1- \sum\nolimits_{i=1}^{k} \mu_j$ where, $\mu_j$ is top $j^{th}$ eigenvalue of the matrix $M$. The dual optimization problem for the \ref{Relaxed_Primal}, thus becomes\\
\rule{\columnwidth}{0.5pt}
\vspace{-0.5cm}
\begin{align}
&\underset{\boldsymbol{\lambda},\boldsymbol{\mu}}{\text{Maximize}} \ \ g(\boldsymbol{\lambda},\boldsymbol{\mu}) =1- \sum\nolimits_{j=1}^{k} \mu_j\nonumber \\
&\ \text{subject to }\nonumber\\
& \mu_j \text{ is top $j^{th}$ eigenvalue of } M,\;\forall j=1,\ldots,k\nonumber\\
&\sum\nolimits_{i=1}^{n}\lambda_i = 1\nonumber\\
&\lambda_i \ge 0,\;\forall i =1,\ldots, n
\eqname{(Relaxed Dual)}\label{Dual_Relaxed_Primal}
\end{align} 
\rule{\columnwidth}{0.5pt}
Let $\widehat{d^*}$ be the optimal value of the \ref{Dual_Relaxed_Primal} problem. In what follows, we state a few key observations with regard to the above primal-dual formulation discussed so far. 
%The proof of this lemma has been given in the supplementary material due to the space constraint.
 %--------------------------------------------------------------------------------------------
\begin{lemma}\label{dual_lemma1} For the given \ref{Primal}, \ref{Relaxed_Primal}, and \ref{Dual_Relaxed_Primal} programs, following hold true.
 \begin{enumerate}[label=(\Alph*)]
 \item $\widehat{d^*} \le \widehat{p^*} \le p^* \le 1$
 \item If $\left(\boldsymbol{\lambda}, \boldsymbol{\mu}\right)$ is a feasible solution of \ref{Dual_Relaxed_Primal}, then
 \begin{eqnarray*}
 0 & \le & \mu_j,\;\forall j\in [k]\\
 0 &\le& \sum\nolimits_{j=1}^{k} \mu_k \le Tr(M) =\sum\nolimits_{i=1}^n \lambda_i=1
 \end{eqnarray*}
 \item $\text{Rank}(M)\le \text{Rank}(\mathbf{X}^{\top}\mathbf{X})=\text{Rank}(\mathbf{X})$
 \item Let $(\boldsymbol{\lambda}^*,\boldsymbol{\mu}^*)$ be the point of optimality for \ref{Dual_Relaxed_Primal} problem. Then top-$k$ eigenvectors $\boldsymbol{v}_1^*,\ldots,\boldsymbol{v}_k^*$ of the matrix $M=\sum_{i=1}^{n}\lambda_i^*\boldsymbol{x}_i\boldsymbol{x}_i^{\top}=\boldsymbol{\lambda}^* \mathbf{X}^{\top}\mathbf{X}$ satisfy the following properties.
\begin{enumerate}
\item These vectors minimize the Lagrangian function $L(\boldsymbol{v}_1,\ldots,\boldsymbol{v}_k,\;\text{\LARGE{$\epsilon$}},\; \lambda_1^*,\ldots,\lambda_n^*,\mu_1^*,\ldots,\mu_k^*)$.
\item These vectors form a feasible solution for both \ref{Relaxed_Primal} and \ref{Primal} problems thus allowing us to use vectors obtained from the \ref{Dual_Relaxed_Primal} as approximate solutions of the \ref{Primal}.
\item Let $\text{\LARGE{$\epsilon$}}_{ALG}$ be the \ref{Relaxed_Primal} objective function value (which is also the value for the \ref{Primal} objective function) corresponding to the feasible solution  $\boldsymbol{v}_1^*,\ldots,\boldsymbol{v}_k^*$ then we must have $p^* \le \text{\LARGE{$\epsilon$}}_{ALG} \le 1$.
\end{enumerate}	   
\end{enumerate}
\end{lemma}
 %--------------------------------------------------------------------------------------------
\begin{proof}
\hfill{}\\
{\bf Part (A):} 
\begin{comment}
To prove the first inequality in part (A), observe that matrix $\mathbf{M}$ is a symmetric PSD matrix and hence we must have $\mu_j \ge 0,\;\forall j=1,\ldots,d$. From the expression (\ref{upper_bound_eigenvalues_sum}) and the fact that $\mu_1,\ldots,\mu_k$ are top-$k$ eigenvalues of a symmetric PSD matrix, we can write the following inequality which follows from the fact that average of top-$k$ numbers (out of $n$ given numbers) is at least as high as average of all the $n$ numbers. 
\begin{eqnarray*}
&& 0 \le \frac{k}{d} \le \sum_{j=1}^{k} \mu_j \\
\Rightarrow && \widehat{d^*} = 1 -\sum_{j=1}^{k} \mu_{j}^{*} \le 1-\frac{k}{d} 
\end{eqnarray*}
This proves the first inequality of part (A). 
\end{comment}
The inequalities follow from weak duality theorem and the fact that $\widehat{p^*}$ is the optimal solution of the (Relaxed Primal) problem, whereas $p^*$ is the optimal solution of the (Primal) problem. The last inequality follows from Lemma \ref{lemma1}. \\\\
{\bf Part (B):} Let $(\boldsymbol{\lambda}, \boldsymbol{\mu})$ be a feasible solution for (Relaxed Dual) problem then by Lemma \ref{dual_lemma}, we can claim that $\mu_j \ge 0$ because $\mu_j$ must be an eigenvalue of the matrix $\mathbf{M}$ and this matrix is always a positive semidefinite. Further, notice that
\begin{align*}
& Tr(\mathbf{M}) = Tr(\sum_{i=1}^{n}\lambda_i\boldsymbol{x}_i\boldsymbol{x}_i^{\top})\\
& = \sum_{i=1}^{n}\lambda_i \; Tr(\boldsymbol{x}_i\boldsymbol{x}_i^{\top})=\sum_{i=1}^{n}\lambda_i Tr(\boldsymbol{x}_i^{\top}\boldsymbol{x}_i)= \sum_{i=1}^n \lambda_i =1
\end{align*}
where, last part of the equation follows from that fact that vectors $\boldsymbol{x}_i$ are unit vectors. Further, if $(\boldsymbol{\lambda},\boldsymbol{\mu})$ is a feasible solution for (Relaxed Dual) then we must also have
\begin{eqnarray}
\sum_{j=1}^{k} \mu_j \le \sum_{j=1}^{d} \mu_j = Tr(\mathbf{M}) =1 \label{upper_bound_eigenvalues_sum}
\end{eqnarray}
where, $\mu_{(k+1)},\ldots,\mu_d$ are the bottom $(d-k)$ eigenvalues of the matrix $M$.  This proves the part (B) of the lemma.\\\\
{\bf Part (C):} This part follows from the standard results in linear algebra.\\\\
{\bf Part (D):}  Let $(\boldsymbol{\lambda}^*,\boldsymbol{\mu}^*)$ be the point of optimality for (Relaxed Dual) problem. Let $\boldsymbol{v}_1^*,\ldots,\boldsymbol{v}_k^*$ be the top-$k$ eigenvectors of the matrix $\mathbf{M}=\sum_{i=1}^{n}\lambda_i^*\boldsymbol{x}_i\boldsymbol{x}_i^{\top}=\boldsymbol{\lambda}^* \mathbf{X}^{\top}\mathbf{X}$. Because $(\boldsymbol{\lambda}^*,\boldsymbol{\mu}^*)$  is an optimal solution for (Relaxed Dual) problem, it must be a feasible solution also for the same problem. This would mean that $\boldsymbol{\mu}_j^*,\;\forall j\in[k]$ must be top-$j^{th}$ eigenvalue of the matrix $\mathbf{M}=\sum_{i=1}^{n}\lambda_i^*\boldsymbol{x}_i\boldsymbol{x}_i^{\top}$. Therefore, by Lemma \ref{dual_lemma}, we can say that the vectors $\boldsymbol{v}_1^*,\ldots,\boldsymbol{v}_k^*$ must minimize the Lagrangian function $L(\boldsymbol{v}_1,\ldots,\boldsymbol{v}_k,\;Z,\; \lambda_1^*,\ldots,\lambda_n^*,\mu_1^*,\ldots,\mu_k^*)$. The feasibility of the vectors $\boldsymbol{v}_1^*,\ldots,\boldsymbol{v}_k^*$ for (Primal) and (Relaxed Primal) problems is trivial due to the fact these vectors are orthonormal basis vectors. The first part of the inequality $p^* \le \text{\LARGE{$\epsilon$}}^* \le 1$ is trivial because $p^*$ is optimal. The second part of this inequality follows from the second inequality given in part (B) of the this lemma.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------------------Duality Gap-------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Approximate Solution of \ref{Primal} Problem} 
Recall that \ref{Primal} is a non-convex optimization problem and hence, in this paper, our approach to solve this problem approximately is as follows.\\
\rule{\columnwidth}{1pt}  
\begin{enumerate}
\item We first find an optimal solution $(\boldsymbol{\lambda}^*,\boldsymbol{\mu}^*)$ for \ref{Dual_Relaxed_Primal} problem. 
\item Next, we find the top-$k$ eigenvectors $\boldsymbol{v}_1^*,\ldots,\boldsymbol{v}_k^*$ of $M=\sum_{i=1}^{n}\lambda_i^*\boldsymbol{x}_i\boldsymbol{x}_i^{\top}$ and treat them as an approximate solution for the original \ref{Primal} problem. Note, these eigenvectors constitute a feasible solution for the \ref{Primal} as well as \ref{Relaxed_Primal} problems (as shown in Lemma \ref{dual_lemma1}). 
\end{enumerate}
\rule{\columnwidth}{1pt} 
In this section, we try to develop an initial theoretical bound on the quality of such an approximate solution for the original \ref{Primal}. For this, note that 
%Recall, \ref{Relaxed_Primal} problem is a non-convex optimization problem and hence it is quite possible that the duality gap (given by $\widehat{p^*}-\widehat{d^*}$) is not zero. Therefore, if we solve the original \ref{Primal} problem by means of solving \ref{Dual_Relax_Primal}, it is possible that . In this section, we identify the conditions under which duality gap for the  \ref{Relaxed_Primal} problem is zero. This will pave the way for our proposed algorithm in the next section.
 %--------------------------------------------------------------------------------------------
%\begin{theorem} 
%\end{theorem}
 %--------------------------------------------------------------------------------------------
%{\bf Proof:} 
%Suppose  $(\boldsymbol{\lambda}^*,\boldsymbol{\mu}^*)$ is a point of optimality for \ref{Dual_Relaxed_Primal} problem. In this case, as per Lemma \ref{dual_lemma1}, we can write down following facts.
%\begin{itemize}
%\item $\mu_j^*,\; \forall j \in [k]$ are top-$k$ eigenvalues of the matrix $M=\sum_{i=1}^{n}\lambda_i^*\boldsymbol{x}_i\boldsymbol{x}_i^{\top}$.
%\item The corresponding eigenvectors  $\boldsymbol{v}_1^*,\ldots,\boldsymbol{v}_k^*$ form a feasible solution for both \ref{Relaxed_Primal} as well as \ref{Primal} problems.
%\end{itemize}
%Now observe that 
the objective function value for both \ref{Relaxed_Primal} and \ref{Primal} problems is identical for the feasible solution $(\boldsymbol{v}_1^*,\ldots,\boldsymbol{v}_k^*)$. Moreover, this value is given by $\text{\LARGE{$\epsilon$}}_{ALG}=\underset{i=1,\ldots,n}{\max} \phi_i$, where $\phi_i=1-\lVert {\mathbf{V}^*} ^{\top} \boldsymbol{x}_i\rVert_2^2$ and $\mathbf{V}^*$ is a matrix comprising vectors   $\boldsymbol{v}_1^*,\ldots,\boldsymbol{v}_k^*$ as its columns.  
\begin{comment}
By making use of use of claim given in part (A) of lemma \ref{dual_lemma1}, we can write that
\begin{eqnarray}
0\le \frac{k}{d}\le \widehat{d^*} \le \widehat{p^*} \le p^* \le \text{\LARGE{$\epsilon$}}^* \le 1
\end{eqnarray}
Therefore, we can measure the approximation quality for the proposed solution of \ref{Primal} problem by the quantity $\text{\LARGE{$\epsilon$}}^*-p^*$ and which can be bounded as follows
\begin{eqnarray}
(\text{\LARGE{$\epsilon$}}^*-p^*) \le  (\text{\LARGE{$\epsilon$}}^* - \widehat{d^*}) \le 1-\frac{k}{d}
\end{eqnarray}
Also, note that 
\end{comment}
The optimal objective function value for \ref{Dual_Relaxed_Primal} would be $\widehat{d^*}=1-\sum_{j=1}^{k}\mu_j^*$. 
By making use of the above facts, we can now write
\begin{align}
& \widehat{d^*}=1-\sum\nolimits_{j=1}^{k}\mu_j^* = 1- \sum\nolimits_{j=1}^{k} {\boldsymbol{v}_j^*}^{\top} M \boldsymbol{v}_j^*\nonumber\\
&=1- \sum\nolimits_{i=1}^{n}\lambda_i^*\sum\nolimits_{j=1}^{k} {\boldsymbol{v}_j^*}^{\top} \boldsymbol{x}_i\boldsymbol{x}_i^{\top}  \boldsymbol{v}_j^* = 1- \sum\nolimits_{i=1}^{n}\lambda_i^* (1-\phi_i)\nonumber\\
&= \sum\nolimits_{i=1}^{n}\lambda_i^*\phi_i \le \underset{i=1,\ldots,n}{max} (\phi_i)= \text{\LARGE{$\epsilon$}}_{ALG}
\end{align}
where, we have made use of the fact that $\sum_{i=1}^{n}\lambda_i^*=1$ and $\lambda_i^* \ge 0,\;\forall i\in[n]$. By using above relation and Lemma \ref{dual_lemma1}, we can say that 
\begin{align*}
&(\text{\LARGE{$\epsilon$}}_{ALG}-p^*) \le  (\text{\LARGE{$\epsilon$}}_{ALG} - \widehat{d^*}) = \left( \underset{i=1,\ldots,n}{max} (\phi_i) - \sum\nolimits_{i=1}^{n}\lambda_i^*\phi_i \right)
\end{align*}
\begin{comment}
Comparing with the previous inequality, we can say that 
\begin{align*}
& (\text{\LARGE{$\epsilon$}}_{ALG}-p^*) \le  (\text{\LARGE{$\epsilon$}}_{ALG} - \widehat{d^*}) \\
& \le \min\left(\left(1-\frac{k}{d}\right),\left(\underset{i=1,\ldots,n}{max} (\phi_i) - \sum_{i=1}^{n}\lambda_i^*\phi_i\right)\right)
\end{align*}
\end{comment}
The above inequality bounds the gap between the primal objective value corresponding to our approximate solution and the unknown optimal primal objective value. Note that the upper bound can be calculated by solving the Relaxed dual. The above inequality also suggests that our approximate solution would indeed be an optimal solution for \ref{Primal} problem whenever we have $\phi_1=\phi_2=\ldots=\phi_n$. In this case, the length of projection any ways would be the same for all the data points when projected into the space spanned by $\boldsymbol{v}_1^*,\ldots,\boldsymbol{v}_k^*$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------------------Min-Max PCA-------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}

\section{Dual Ascent Method}
In this section, we present a dual ascent method to solve the \ref{Dual_Relaxed_Primal} problem. The high level idea behind dual ascent algorithm is given as follows\\
\hrule
\begin{enumerate}
\item Assign $t \leftarrow 0$.
\item Start with an initial vector $\boldsymbol{\lambda}^{(0)} \in \mathbb{R}^n$ such that it satisfies last two constraints of the \ref{Dual_Relaxed_Primal} problem. That is  $\boldsymbol{\lambda}^{(0)} \in \mathbb{R}^n$ is a valid probability distribution. 
\item Compute a vector $\boldsymbol{\mu}^{(0)}\in \mathbb{R}_{+}^{k}$ such that they form the top-k eigenvalues of the matrix $M(\boldsymbol{\lambda}^{(0)})=\sum_{i=1}^{n}\lambda_i^{(0)}\boldsymbol{x}_i\boldsymbol{x}_i^{\top}$.
\item Find an ascent direction $\boldsymbol{d}^{(t)} \in \mathbb{R}^n$ for $\boldsymbol{\lambda}^{(t)}$.
\begin{enumerate}
\item If there is no ascent direction then stop.
\item Otherwise, move an appropriate step length along the ascent direction such that $\boldsymbol{\lambda}^{(t+1)} \leftarrow \boldsymbol{\lambda}^{(t)} + \boldsymbol{d}^{(t)}$ is still a valid probability distribution and moreover, the dual objective function value at $\boldsymbol{\lambda}^{(t+1)}$ is more than the value at $\boldsymbol{\lambda}^{(t)}$. Assign $t \leftarrow (t+1)$ and go back to step 3 above.  
\end{enumerate}
\end{enumerate}
\hrule
Note that in the above procedure, following two steps are crucial and require further elaboration - (i) finding an ascent direction $\boldsymbol{d}^{(t)} $, (ii) finding an appropriate step length $\alpha_t>0$. 
\subsection{Finding an Ascent Direction} In order to find an ascent direction, let us define the following function (inspired from \ref{Dual_Relaxed_Primal} problem) for any $\boldsymbol{\lambda}\in \mathbb{R}_{+}^n$ in the probability simplex. 
\begin{eqnarray}
f(\boldsymbol{\lambda})=1-\sum_{j=1}^{k} \mu_j
\end{eqnarray}
where $\mu_j$ is the top $j^{th}$ eigenvalue of the matrix $M(\boldsymbol{\lambda})=\sum_{i=1}^{n}\lambda_i \boldsymbol{x}_i^{\top}\boldsymbol{x}_i$. In light of this definition, we can say that a direction ${\boldsymbol{d}}^{(t)}=[d_1^{(t)},\ldots, d_n^{(t)}]^{\top}$ is an ascent direction at $\boldsymbol{\lambda}=\boldsymbol{\lambda}^{(t)}$ (assuming it is not the point of local maximum) if it satisfies the following condition.
\begin{eqnarray}
\left[\nabla f\left(\boldsymbol{\lambda}^{(t)}\right)\right]^{\top}{\boldsymbol{d}}^{(t)}=\left[\frac{\partial f\left(\boldsymbol{\lambda}^{(t)}\right)}{\partial \boldsymbol{\lambda}^{(t)}}\right]^{\top}{\boldsymbol{d}}^{(t)} \ge 0
\end{eqnarray}
\begin{lemma}[Gradient] If $\boldsymbol{\lambda}^{(t)}$ is not a point of optimality for the \ref{Dual_Relaxed_Primal} problem then the $\ell^{th}$-coordinate of the gradient vector $\nabla f\left(\boldsymbol{\lambda}^{(t)}\right)$ is given by
\begin{eqnarray}
\frac{\partial f\left(\boldsymbol{\lambda}^{(t)}\right)}{\partial {\lambda}_{\ell}^{(t)}}&=& -\sum_{j=1}^{k} {\boldsymbol{v}_j^{(t)}}^{\top} (\boldsymbol{x}_{\ell}\boldsymbol{x}_{\ell}^{\top})  {\boldsymbol{v}_j^{(t)}}= -\sum_{j=1}^{k} \lVert \boldsymbol{x}_{\ell}^{\top} \boldsymbol{v}_j^{(t)}\rVert^2\\
&=& -\sum_{j=1}^{k} \left(\text{orthogonal projection length of } \boldsymbol{x}_{\ell} \text{ onto the direction } \boldsymbol{v}_j^{(t)}\right)^2,
\end{eqnarray}
where, $\ell =1,\ldots,n$.
\end{lemma}
{\bf Proof:} Note that the gradient vector $\nabla f\left(\boldsymbol{\lambda}^{(t)}\right)$ would be given by  
\begin{eqnarray}
\frac{\partial f\left(\boldsymbol{\lambda}^{(t)}\right)}{\partial \boldsymbol{\lambda}^{(t)}}= \left[\frac{\partial (1-\sum_{j=1}^{k} \mu_j^{(t)})}{\partial \boldsymbol{\lambda}^{(t)}}\right]
\end{eqnarray}
The ${\ell}^{th}$ coordinate of this ascent direction can be given as follows
\begin{eqnarray}
\frac{\partial f\left(\boldsymbol{\lambda}^{(t)}\right)}{\partial {\lambda}_{\ell}^{(t)}} = - \left[\frac{\partial (\sum_{j=1}^{k} \mu_j^{(t)})}{\partial {\lambda}_{\ell}^{(t)}}\right], \;\forall {\ell}=1,2\ldots,n.
\end{eqnarray}
Let $\boldsymbol{v}_1^{(t)}, \ldots \boldsymbol{v}_k^{(t)}$ are the top-$k$ eigenvectors of the matrix $M(\boldsymbol{\lambda}^{(t)})$ then above equation can be written as
\begin{eqnarray}
\frac{\partial f\left(\boldsymbol{\lambda}^{(t)}\right)}{\partial {\lambda}_{\ell}^{(t)}} = - \left[\frac{\partial (\sum_{j=1}^{k} {\boldsymbol{v}_j^{(t)}}^{\top}M(\boldsymbol{\lambda}^{(t)})\boldsymbol{v}_j^{(t)}))}{\partial {\lambda}_{\ell}^{(t)}}\right]
\end{eqnarray}
Recall that
\begin{eqnarray}
M(\boldsymbol{\lambda}^{(t)}) &=& \sum_{i=1}^{n}\lambda_i^{(t)}\boldsymbol{x}_i\boldsymbol{x}_i^{\top}
\end{eqnarray}
Substituting this expression for $M(\boldsymbol{\lambda}^{(t)})$ in the previous equation give us the following relation.
\begin{eqnarray}
\frac{\partial f\left(\boldsymbol{\lambda}^{(t)}\right)}{\partial {\lambda}_{\ell}^{(t)}} &=& -\sum_{j=1}^{k} {\boldsymbol{v}_j^{(t)}}^{\top} (\boldsymbol{x}_{\ell}\boldsymbol{x}_{\ell}^{\top})  {\boldsymbol{v}_j^{(t)}} - 2\sum_{j=1}^{k} \sum_{i=1}^{n}\lambda_i^{(t)}  \left(\frac{\partial \boldsymbol{v}_j^{(t)}}{\partial \lambda_{\ell}^{(t)}}\right)^{\top}(\boldsymbol{x}_{i}\boldsymbol{x}_{i}^{\top})\boldsymbol{v}_j^{(t)}\\
&=& -\sum_{j=1}^{k} {\boldsymbol{v}_j^{(t)}}^{\top} (\boldsymbol{x}_{\ell}\boldsymbol{x}_{\ell}^{\top})  {\boldsymbol{v}_j^{(t)}} - 2\sum_{j=1}^{k} \left(\frac{\partial \boldsymbol{v}_j^{(t)}}{\partial \lambda_{\ell}^{(t)}}\right)^{\top}M(\boldsymbol{\lambda}^{(t)})\boldsymbol{v}_j^{(t)}\\
&=& -\sum_{j=1}^{k} {\boldsymbol{v}_j^{(t)}}^{\top} (\boldsymbol{x}_{\ell}\boldsymbol{x}_{\ell}^{\top})  {\boldsymbol{v}_j^{(t)}} - 2\sum_{j=1}^{k} \mu_j^{(t)}\left(\frac{\partial \boldsymbol{v}_j^{(t)}}{\partial \lambda_{\ell}^{(t)}}\right)^{\top}\boldsymbol{v}_j^{(t)}
\end{eqnarray}
The last term in the above expression would be zero because of the fact that
\begin{eqnarray}
\left(\frac{\partial \boldsymbol{v}_j^{(t)}}{\partial \lambda_{\ell}^{(t)}}\right)^{\top}\boldsymbol{v}_j^{(t)}=0,\;\forall j=1,\ldots, k;\;\forall \ell=1,\ldots,n
\end{eqnarray}
This facts follows from the another fact that $\boldsymbol{v}_j^{(t)},\;\forall j=1,\ldots,k$ are eigenvectors and hence we must have ${\boldsymbol{v}_j^{(t)}}^{\top}\boldsymbol{v}_j^{(t)}=1$. Now differentiating this relation on both the sides with respect to $\lambda_{\ell}$ would give us the desired fact.

\end{comment}
 
\begin{comment}


\subsection{Deciding Step Size }
In order to decide the step size, we need to move only that much distance along the ascent direction so that (i) feasibility of $\boldsymbol{\lambda}^{(t+1)}$ gets maintained, and (ii) $f(\boldsymbol{\lambda}^{(t+1)}) \ge f(\boldsymbol{\lambda}^{(t)})$. We can achieve this by solving the following program
\begin{equation}
\begin{aligned}
& \underset{d_1,d_2,\ldots,d_n}{\text{Maximize}} && \sum_{\ell=1}^{n} \frac{\partial f(\boldsymbol{\lambda}^{(t)})}{\partial \lambda_{\ell}^{(t)}}d_{\ell} =\sum_{\ell=1}^{n} \alpha_{\ell}\;d_{\ell} \\
& \text{subject to}
& & 0 \le \lambda_{\ell}^{(t)}+d_{\ell} \le 1,\;\forall \ell=1,\ldots,n\\
& & &\sum_{\ell=1}^{n}d_{\ell} = 0\\
& & & -\frac{\epsilon}{\sqrt{n}} \le d_{\ell} \le \frac{\epsilon}{\sqrt{n}},\;\forall \ell=1,\ldots,n 
\end{aligned} \eqname{(LP)} \label{LP}
\end{equation} 
A few remarks are in order with regard to the above program
\begin{itemize}
\item For a given data set and current estimate $\boldsymbol{\lambda}^{(t)}$, the above program is an LP in $d_1,\ldots,d_n$.
\item The first two constraint ensure that  $\boldsymbol{\lambda}^{(t)}+\boldsymbol{d}$ is a valid probability distribution.
\item The last constraint involves a constant $0 \le\epsilon <1$ and it restricts the movement of $\boldsymbol{\lambda}^{(t)}$ because otherwise the corresponding ascent direction may no more be an ascent direction.
\item Choice of $\epsilon$ is crucial here. Too low value for $\epsilon$ may not give much increase in the objective function value. On the other hand, a too high value for $\epsilon$ may result in function value $f(\cdot)$ lower than the current value. One of the guiding principle behind $\epsilon$ value is that the corresponding optimal objective function value of the above LP must be nonnegative. If we find the optimal value of the above LP as negative then we need to reduce the value of $\epsilon$. For this, we start with $\epsilon=0.1$ and reduce it by half until the answer of LP is a non-negative value. 
\end{itemize}
The above LP can be written into the following equivalent form.
\begin{equation}
\begin{aligned}
& \underset{d_1,d_2,\ldots,d_n}{\text{Maximize}} && \sum_{\ell=1}^{n} \alpha_{\ell}\;d_{\ell} \\
& \text{subject to}
& & \sum_{\ell=1}^{n}d_{\ell} = 0\\
& & & - \min \left(\frac{\epsilon}{\sqrt{n}}, \lambda_{\ell}\right) \le d_{\ell} \le \min\left(\frac{\epsilon}{\sqrt{n}}, 1-\lambda_{\ell}\right),\;\forall \ell=1,\ldots,n
\end{aligned} \eqname{(LP1)} \label{LP1}
\end{equation} 

\end{comment}

